New Wide Locally Recoverable Codes with Unified Locality

Wide Locally Recoverable Codes (LRCs) have recently been proposed as a solution for achieving high reliability, good performance, and ultra-low storage cost in distributed storage systems. However, existing wide LRCs struggle to balance optimal fault tolerance and high availability during frequent system events. By analyzing the existing LRCs, we reveal three limitations in the LRC construction which lay behind the non-optimal overall performance from multiple perspectives, including non-minimum local recovery cost, non cluster-topology-aware data distribution, and non XOR-based local coding. Thanks to the flexible design space offered by the locality property of wide LRCs, we present UniLRC, which unifies locality considerations in code construction. UniLRC achieves the optimal fault tolerance while overcoming the revealed limitations. We implement UniLRC prototype and conduct comprehensive theoretical and system evaluations, showing significant improvements in reliability and performance over existing wide LRCs deployed in Google and Azure clusters.

==> sections/implementation.tex <==
\section{Implementation}
UniLRC is implemented on HDFS 3.0.

==> sections/related_work.tex <==
\section{Related Work}
% LRCs have widely studied and deployed in the last decade due to their practical improvements over MDS codes.
% Microsoft Azure and Facebook first published the commercial use of LRCs \cite{huang2012erasure,asteris2013xoring} industry.
% Then, there are many academic research for finding LRC construction from many scenes \cite{cadambe2013upper,gopalan2012locality,agarwal2018combinatorial,barg2017locally,papailiopoulos2014locally,tamo2014bounds,tamo2016bounds}.
% One area of research has been explicit constructions of distance optimal codes \cite{barg2017locally,haymaker2018locally,liu2017new,luo2021constructions,micheli2019constructions,tamo2014family,tamo2016optimal}.
% Tamo and Barg \cite{zhang2020new} were among the first to provide a general construction of distance-optimal LRCs (with small field sizes), but with some constraints on the allowable parameters.
% This construction was further generalized by Kolosov et al. \cite{kolosov2020fault} for a wide range of parameters. Recent years have seen a surge in research on MR-LRCs \cite{balaji2015partial,barg2022construction,cai2021construction,gopalan2017maximally,gopalan2014explicit,gopi2020maximally,gopi2022improved,grezet2019uniform,guruswami2020ϵ}. Recently, Gopi et al. \cite{gopi2022improved} provided an explicit construction of MR-LRCs which is broad.
% Another area of research is $(r, \delta)$-LRC \cite{zhang2020new,cai2020optimal,kong2021new},  was introduced by Prakash et al. \cite{prakash2012optimal} for tolerating $\delta-1$ failure in one local group. 
% However, this body of work fails to meet the multifaceted demands of wide codes in large-scale storage systems.

\textbf{Wide codes.} Wide codes are known to be deployed in the commercial settings, Backblaze \cite{Backblaze}, VAST \cite{VAST} and Google \cite{kadekodi2023practical}.
The VAST \cite{VAST} has reported a codelength of $154$ in their cluster deployment. 
Kadekodi et al. \cite{kadekodi2023practical} has shown that subtle factors can affect wide LRC reliability in real Google storage clusters, and also give the particularly useful settings for applications, i.e., the field size (search-space for coefficients to construct the LRC) is fixed to be $256$, n is between $25-150$, and the rate of the code is at least $0.85$ (i.e. storage overhead is at most $1.17 \times$ and $l < k$).
%
The recent works have studied wide LRC in academia \cite{hu2021exploiting}.
The study \cite{li2017facilitating} uses local erasure codes
with width $1024$ in hard disks for the read-retry problem and
the study \cite{haddock2019high} utilizes GPUs to boost the encoding/decoding performance of wide stripes.
Hu et al. \cite{hu2021exploiting} study the performance issues in repair, encoding, and update performance of wide LRC.  
XHR-Code utilizes a triple dimensional framework to place more chunks within rack for decreasing the cross-rack overhead under failure recovery \cite{yang2022xhr}.
Some work have study how to efficiently merge old stripes into a new wide LRC stripe \cite{wu2024optimal,wu2022optimal}.
Our work is the first to give new constructions of wide LRC
from a unified performance consideration on normal read, 
degraded read and reconstruction.


\textbf{Locality in erasure coding.} 

% The code designs for rack-level are known in recent years \cite{wang2023rack,yang2024transformation,chen2019explicit,yang2024construction,zhou2022rack}. The papers focus on the low cross-rack access on recovery via constructing the special codes, e.g., RS \cite{yang2024transformation}, MSR \cite{wang2023rack,chen2019explicit,zhou2022rack} and locally repairable array codes \cite{yang2024construction}.
% % [TODO: NEED TO EXPLAIN, GIVEN A TABLE LIST].
% LRC shows good performance in wide codes scenes. 
% We list the main results of cluster-aware LRC as Table \ref{tab:comparison}.
% Hu et al. \cite{hu2021exploiting} is first to study the wide LRC in research and bring low cost on storage cost and cross-cluster traffic of recovery and update, but they do not optimize the cross-cluster traffic into the minimizing, i.e, $0$ cross cluster access in single failure. 
% \cite{cai2024repairing} and \cite{10619677} focus on a high reliability systems with tolerating more than one cluster failed or the failure number exceeds the locality.
% Cai et al. \cite{cai2024repairing} provides a repairing schemes for Tamo-Barg codes \cite{tamo2014family}, and the main objects to optimize the one failed rack and exclude the locality of local groups.
% \cite{10619677} provides a new construction of LRC for optimal repair bandwidth with the number of failures exceeds the locality.
% \cite{yang2022xhr} provides a new RS like code called XOR-Hitchhiker-RS (XHR) code, to decrease the
% cross-rack overhead and still maintain low storage cost. The key idea of XHR is that it utilizes a triple dimensional framework to place more chunks within racks and reduce global repair triggers.
% Our work focus on both normal and recovery performance in practically large-scale storage systems, and achieve the optimal \textit{uniform access}, \textit{file access} and \textit{cluster access}.
